DDS: Decoupled Dynamic Scene-Graph Generation Network

Scene-graph generation involves creating a structural representation of the relationships between objects in a scene by predicting subject-object-relation triplets from input data. Existing methods show poor performance in detecting triplets outside of a predefined set, primarily due to their reliance on dependent feature learning. To address this issue, we propose DDS -- a decoupled dynamic scene-graph generation network -- that consists of two independent branches that can disentangle extracted features. The key innovation of the current paper is the decoupling of the features representing the relationships from those of the objects, which enables the detection of novel object-relationship combinations. The DDS model is evaluated on three datasets and outperforms previous methods by a significant margin, especially in detecting previously unseen triplets.

==> contents/0.abstract.tex <==
\begin{abstract}
Scene-graph generation involves creating a structural representation of the relationships between objects in a scene by predicting subject-object-relation triplets from input data. Existing methods show poor performance in detecting triplets outside of a predefined set, primarily due to their reliance on dependent feature learning. To address this issue we propose DDS-- a decoupled dynamic scene-graph generation network-- that consists of two independent branches that can disentangle extracted features. The key innovation of the current paper is the decoupling of the features representing the relationships from those of the objects, which enables the detection of novel object-relationship combinations. The DDS model is evaluated on three datasets and outperforms previous methods by a significant margin, especially in detecting previously unseen triplets. 

 %We also conduct an ablation study to evaluate the performance of individual components of our proposed architecture.
\end{abstract}

==> contents/1.introduction.tex <==
\section{Introduction}
Dynamic Scene-Graph (DSG) provides a graph structure presenting the relationships among different objects in a scene by predicting relationship triplets composed of $\langle subject, object, relationship \rangle$ at each frame of an input video. This acts as a foundational block for various computer vision tasks\cite{ulutan2020actor, liu2019caesar}. Current DSG generation systems~\cite{ji2021detecting, li2022dynamic, cong2021spatial} have poor performance when facing a triplet that was not present during training, even though the individual components have been seen. However, in a more realistic deployment scenario, the network will likely encounter triplets that it has not seen before. Therefore, a system should be able to transfer the learned concepts of relationships and objects to compose unseen triplets. This poor performance is mainly attributed to the learning of highly dependent feature representations of relationships and objects. The proposed decoupled dynamic scene-graph (DDS) addresses this issue. %To improve on this, this paper introduces DDS - Dynamic Decoupled Scene-Graph generation network. %to deal with the  mentioned limitation. 

Fig. \ref{fig:concept} shows the core idea of the proposed DDS network. This architecture utilizes two different branches to learn decoupled features for relationships and objects. As shown in the figure, DDS learns the concept of `ride', `on', `person', `bicycle', and `bed' from the training examples of a `person riding a bike' and a `dog on the bed' independently. The decoupled design makes DDS look into different spatial regions for relationships and objects. These learned concepts are transferred to successfully detect the unseen triplet $\langle dog, bicycle, ride \rangle$.
% , see Section~\ref{sec:qual} for more details.
%TODO Put this back

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/DDS1_2.jpg}
\end{center}
\vspace{-0.4cm}
\caption{Diagram to show the concept learning and transferring in DDS. By focusing on different spatial regions, DDS learns the concept of relationships (ride, on) and objects (person, bicycle, bed) independently.
}
\label{fig:concept}
\vspace{-0.2cm}
\end{figure} 

% Existing works~\cite{ji2021detecting, li2022dynamic, cong2021spatial} for generating DSGs follow a two-stage process. First, an object detector localizes objects irrespective of their relationship status. In the second stage, different attention-based~\cite {ji2021detecting, li2022dynamic} and graph-based~\cite {cong2021spatial} methods utilize features extracted from the previously localized objects to predict relationships. In this process, the extracted features of the objects are fed throughout the network for relationship detection. As a result, these methods learn to associate a relationship only with a particular combination of objects and hence perform poorly in predicting unseen triplets. %Moreover, relying on off-the-shelf object detectors reduces the generic learning capability of the models\cite{iftekhar2022look}. 

% In contrast, 
DDS ensures the learning of discriminative spatio-temporal cues for relationships and objects. Fig. \ref{fig:model_architecture} shows the overview of our architecture. It consists of two separate branches: the relation and the object branch. We chose a transformer-based encoder-decoder \cite{carion2020end} architecture for these branches with two different sets of queries. Moreover, a novel temporal decoder is added to embed temporal information into the queries. These separate sets of queries focus on learning generalized representations for relationships and objects from differently encoded feature maps in both temporal and spatial domains. This is significantly better than the existing works, where the same object features are used for both object and relationship detection. Also, DDS does not have the dependence on off-the-shelf object detectors like previous works.
 
 Our proposed model is thoroughly evaluated on the Action-Genome\cite{ji2020action} dataset for DSG generation, where it achieves significant performance gains compared to the SOTA models. Additionally, we evaluate DDS on the task of static scene-graph (SSG) generation on the HICO-DET\cite{chao2018learning} dataset and unusual SSG generation on the UnRel\cite{peyre2017weakly} dataset, where DDS outperforms all the existing models in both datasets. Finally, the proposed design choices are evaluated in an extensive ablation study. 


==> contents/tables.tex <==



%\section{tables \& stuff}














% \begin{table}[h]
% \centering
% \adjustbox{width=0.8\columnwidth}{

% \begin{tabular}{ccc}
% \hline
% \begin{tabular}[c]{@{}c@{}}Number of \\ Queries, $N_{q}$\end{tabular} & Unseen (mAP)  & Seen (mAP)    \\ \hline
% 32                                                                    & 19.8          & 30.5          \\
% 64                                                                    & \textbf{21.1} & \textbf{31.7} \\
% 100                                                                   & 19.7          & 31.3          \\ \hline
% \end{tabular}
% }
% \vspace{0.1cm}
% \caption{DDS's performance with different number of queries, $N_{q}$.}

% \label{tab:ab_hico_query}
% \end{table}




% \large \textbf{Still running on other checkpoints to see if there's better results, weirdly the no Query F is better on the R@100}


% \begin{table}[h]
% \centering
% \adjustbox{width=0.8\columnwidth}{

% \begin{tabular}{cccccc}
% \hline
% O. Query & R. Query & Com. Mem. & R@20 & R@50 & R@100 \\
% \hline

% \cmark         & \xmark      & \xmark         & 7.81                    & 17.68                   & 24.55                    \\
% \xmark        & \cmark       & \xmark         & 8.08                    & 16.14                   & 21.13                     \\
% \cmark         & \cmark       & \xmark         & 9.42                    & 17.65                    & 25.02                     \\
% \cmark         & \cmark       & \cmark          & 5.928                    & 15.97                    & 22.77                        \\
% \hline
% \end{tabular}
% }
% \vspace{0.1cm}
% \label{tab:ab_AG_query}
% \caption{Ablations for AG - different query forward methods - Unseen triplets}
% \end{table}

%\xmark        & \xmark      & \xmark         & 4.24                     & 16.021                   & 26.06                     \\






% \begin{table}[h]
% \centering
% \adjustbox{width=0.8\columnwidth}{
% \begin{tabular}{lcccc}
%                   & \multicolumn{1}{l}{Seen} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{Unseen} & \multicolumn{1}{l}{} \\ \hline
%                   & R@20                     & R@50                 & R@20                       & R@50                 \\ \hline
% STTran            & 33.69                    & 36.59                & 0.2976                     & 4.38                 \\
% DDS + O. Query    & 40.89                    & 48.65                & 7.81                       & 17.68                \\
% DDS + V. Query    & 40.08                    & 48.15                & 8.08                       & 16.14                \\
% DDS + O. V. Query & 40.88                    & 48.79                & 9.42                       & 17.65    \\ \hline           
% \end{tabular}
% }
% \vspace{0.1cm}
% \caption{Comparison between DDS and STT using the proposed compositional split.}
% \label{tab:dds_stt}
% \end{table}


